Federated Few-Shot Learning for Mobile NLP

Natural language processing (NLP) sees rich mobile applications. To support various language understanding tasks, a foundation NLP model is often fine-tuned in a federated, privacy-preserving setting (FL). This process currently relies on at least hundreds of thousands of labeled training samples from mobile clients; yet mobile users often lack willingness or knowledge to label their data. Such an inadequacy of data labels is known as a few-shot scenario; it becomes the key blocker for mobile NLP applications. For the first time, this work investigates federated NLP in the few-shot scenario (FedFSL). By retrofitting algorithmic advances of pseudo labeling and prompt learning, we first establish a training pipeline that delivers competitive accuracy when only 0.05% (fewer than 100) of the training data is labeled and the remaining is unlabeled. To instantiate the workflow, we further present a system FeS, addressing the high execution cost with novel designs. (1) Curriculum pacing, which injects pseudo labels to the training workflow at a rate commensurate to the learning progress; (2) Representational diversity, a mechanism for selecting the most learnable data, only for which pseudo labels will be generated; (3) Co-planning of a model's training depth and layer capacity. Together, these designs reduce the training delay, client energy, and network traffic by up to 46.0$\times$, 41.2$\times$ and 3000.0$\times$, respectively. Through algorithm/system co-design, FFNLP demonstrates that FL can apply to challenging settings where most training samples are unlabeled.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> alg-pacing-bk.tex <==
\begin{algorithm}[t]
	\footnotesize
	\SetAlgoNoEnd
  \SetKwProg{Fn}{Function}{~}{end}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      % Pre-trained model, $\Theta$;\\
      Target accuracy, $acc$;\\
      Initial configuration list, $l$;\\
      Number of candidate configurations, $t$;\\
      AUG-E threshold, $s$;\\
      Trial round, $trial\_round$.
    }

  \Output{
      Fine-tuned model, $\Theta_{i}$~(i=1,2\dots).
      % $Q_b$\;   
    }
  \BlankLine

  \Fn{Cloud\_controller():}{
    Iteration $i$=0;\\
    $l_{win}$, $l_{candidate}$, $i$ $\leftarrow$ Switch($i,l$);\\
    % $Client_{train}$ $\leftarrow$ selects $N$ clients;\\
    % Iteration i=0;\\
      \While{Eval($\Theta_{i}$) $<$ $acc$}
      { 
        Pacing(i, $l_{win}$);\\
        $E$ $\leftarrow$ Compute AUG-E;// accuracy degradation detect\\
        
        \If{$E$<$s$}{
          $l_{win}$, $l_{candidate}$, $i$ $\leftarrow$ Switch($i,l_{candidate}$);\\
        }
        }
        Exit training.
      }

  \Fn{Client\_training(i):}{
    $\Theta_{i}$ $\leftarrow$ Receive global model from cloud;\\
    $\Theta_{i+1}(n)$ $\leftarrow$ Train and update local model; \\
    Send updated model $\Theta_{i+1}(n)$ to cloud.
  }

  \Fn{Client\_labeling(i):}{
    $<f,n,k>$ $\leftarrow$ Receive configuration from cloud;\\
    \If{i\%f==0}{
    $\Theta_{i}$ $\leftarrow$ Receive global model from cloud for inference;\\
    $labels$ $\leftarrow$ Selected pseudo labels for subsequent training.}
  }
  
  \Fn{Pacing(i, $<f,n,k>$):}{
    $Client_{train}$ $\leftarrow$ selects $N$ clients;\\
      Send model $\Theta_{i}$ to $Client_{train}$;\\
      $Client_{label}$ $\leftarrow$ selects $n$ clients;\\
      Send $\Theta_{i}$ and $<f,n,k>$ to $Client_{label}$;\\
      \textbf{Parallel}: Client\_labeling(i), Client\_training(i);\\

      $\Theta_{i+1}(n)$ $\leftarrow$ Receive updated model from $Client_{train}$;\\
      $\Theta_{i+1}$ $\leftarrow$ Fedavg($\Theta^{k}_{i}(n)$);\\
  }

  \Fn{Switch(i, l):}{
    $E_{l}$ $\leftarrow$ []; \# Augment efficiency list\\
    Iteration\_tmp $i_{tmp}$=i;\\
          \For{$<f,n,k> \in l$}{
            \While{$i<i_{tmp} + trial\_round$.}{
              Pacing(i, $<f,n,k>$);\\
              i++;\\
            }
            $E_{l}$ $\leftarrow$ Compute AUG-E;\\
        }
        $l_{win}$ $\leftarrow$ argmax$_{l}$($E_{l}$);\\
        $l_{candidate}$ $\leftarrow$ argmax$_{l}$($E_{l}$, num=t);\\
  }
  
  \caption{Our Pacing Configurator}\label{alg:pacing}
\end{algorithm}


==> alg-planning.tex <==
\begin{algorithm}[t]
	\footnotesize
	\SetAlgoNoEnd
  \SetKwProg{Fn}{Function}{~}{end}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
    Pre-trained model, $\Theta$.
    }

  \Output{
      Number of top layers, $\#top$;\\
      Number of middle layers, $\#mid$;\\
      % $Q_b$\;   
    }
  \BlankLine

  \Fn{Cloud\_controller():}{
    $\#top$ $\leftarrow$ Number of all layers of $\Theta$ ;\\
    acc $\leftarrow$ Fine-tune and eval $\Theta$ with $\#top$; // baseline accuracy\\
    $\#top$, $\#mid$ $\leftarrow$ 0; // initial configuration\\
    \While{Eval($\Theta$) < acc}{
      $\#top$++; \\
      $\Theta$ $\leftarrow$ model fine-tuned with $\#top$; \\
    }
    $\Theta$ $\leftarrow$ fine-tuned with $\#top$-1, $\#mid$+1; // reduce layer capacity\\
    \While{Eval($\Theta$) $\geqq$ acc}{
      $\#top$=$\#top$-1; $\#mid$++;\\
      $\Theta$ $\leftarrow$ model fine-tuned with $\#top$, $\#mid$; \\
    }
  }

  \caption{Our Co-planning Configurator}\label{alg:planning}
\end{algorithm}


==> fig-bkgnd-prompt.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.48\textwidth]{figs/workflow-local-prompt-learning.pdf}
	%  \vspace{-10pt}
	\caption{Workflow of local prompt learning. \cdq{todo: polish this figure}.} 
	% (1) Labeled data are usually sparsely distributed on mobile devices;
	% (2) Pattern encoding some form of task description are created to convert training samples to cloze questions;
	% (3) Client data cannot be transferred, we introduce FL;
	% (4) We propose a novel FL framework, FedPET, to train a model on the client side and transfer the model to the server side for evaluation.
	\vspace{-10pt}
	\label{fig:bkgnd-prompt}
\end{figure}

==> fig-design-bitfit.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/bitfit/agnews.png}
            \subcaption{\texttt{AGNEWS}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/bitfit/mnli.png}
            \subcaption{\texttt{MNLI}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/bitfit/yahoo.png}
            \subcaption{\texttt{YAHOO}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/bitfit/yelp.png}
            \subcaption{\texttt{YELP-F} }
        \end{minipage}
    \end{minipage}
    
    \caption{BitFit + Freeze vs. Freeze.}
    \label{fig:eval-design-bitfit}
    \vspace{-10pt}
\end{figure*}


==> fig-design-overview.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}[b]{1\textwidth}
		\begin{minipage}[b]{0.70\textwidth}
            \includegraphics[width=1\textwidth]{figs/design-workflow.pdf}
            \subcaption{Workflow}
        \end{minipage}
        \begin{minipage}[b]{0.26\textwidth}
            \includegraphics[width=1\textwidth]{figs/design-framework.pdf}
            \subcaption{Framework}
        \end{minipage}
	\end{minipage}
	%  \vspace{-10pt}
	\caption{Overview of \sys.} 
	% \vspace{-15pt}
	\label{fig:design-overview}
\end{figure*}

==> fig-eval-filter.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/ablation/filter/sactter-agnews.pdf}
            \subcaption{\texttt{AGNEWS}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/ablation/filter/sactter-mnli.pdf}
            \subcaption{\texttt{YAHOO}}
        \end{minipage}
    \end{minipage}
    
    \caption{Representative filter outperforms under different filter ratio. \cdq{Change y-axis to log.}}
    \label{fig:eval-eval-filter}
    \vspace{-10pt}
\end{figure}


==> fig-eval-pacing.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/pacing/c0.pdf}
            \subcaption{\texttt{AGNEWS}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/pacing/c1.pdf}
            \subcaption{\texttt{YAHOO}}
        \end{minipage}
    \end{minipage}
    
    \caption{Curriculum pacing and metric AUG-E help we move to the great configuration gradually.}
    \label{fig:eval-eval-pacing}
    \vspace{-10pt}
\end{figure}


==> fig-intro-framework.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.48\textwidth]{figs/intro-framework.pdf}
	%  \vspace{-10pt}
	\caption{Workflow of \sys. \mwx{Not needed?} 
	% (1) Labeled data are usually sparsely distributed on mobile devices;
	% (2) Pattern encoding some form of task description are created to convert training samples to cloze questions;
	% (3) Client data cannot be transferred, we introduce FL;
	% (4) We propose a novel FL framework, FedPET, to train a model on the client side and transfer the model to the server side for evaluation.
	} 
	\vspace{-10pt}
	\label{fig:into-framework}
\end{figure}

==> obsolete/alg-trial.tex <==
\begin{algorithm}
	\footnotesize
	\SetAlgoNoEnd
  \SetKwProg{Fn}{Function}{~}{end}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{MIN}{MIN}\SetKwFunction{MAX}{MAX}\SetKwFunction{LENGTH}{LENGTH}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}\SetKwInOut{Variable}{Variable}

  \Input{
      % Pre-trained model, $\Theta$;\\
      Model capacity threshold, $\varphi $;\\
      Trial interval, $trial\_intvl$;\\
      Start-up depth and width, $D_{0}$ and $W_{0}$;\\
      Step of depth and width, $S_d$ and $S_w$.
    }

  \Output{
      Fine-tuned adapter weights, $\Theta_{i}$~(i=1,2\dots).
      % $Q_b$\;   
    }
  \BlankLine

  \Fn{Cloud\_controller():}{
    $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ $\leftarrow$ selects $3N$ clients;\\
    Iteration i=0;\\
    $T_{trial}$=$T_{now}$;\\
    Dispatch(0); // Init model and trigger client training\\
      \While{Eval() $<$ $acc$}
      { 
        i++;\\
        $\Theta^{k}_{i}(n)$ $\leftarrow$ Receive updated adapters from $Trial_{k}$;\\
      $\Theta^{k}_{i}$ $\leftarrow$ Fedavg($\Theta^{k}_{i}(n)$);\\
      $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ $\leftarrow$ selects $3N$ new clients;\\
        \eIf{$T_{now}$ - $T_{trial}$ > $trial\_intvl$}{Compare accuracy under different $\Theta^{k}_{i}$;\\
        $\Theta_{i}$ $\leftarrow$ Winner track;
        $D_{i}, W_{i}$ $\leftarrow$ Winner setting;\\
        $T_{trial}$=$T_{now}$;\\
        Dispatch(i) // Inherit winner track;\\}{
          Send the aggregated model $\Theta^{k}_{i}$ to $Trial_{k}$.
        }
      }
      Exit training.
    }

  \Fn{Client\_training(i,k):}{
    $\Theta_{i}^{k}$ $\leftarrow$ Receive global adapter  from cloud;\\
    $\Theta_{i+1}^{k}(n)$ $\leftarrow$ Train and update local adapter; \\
    Send updated adapter $\Theta_{i+1}^{k}(n)$ to cloud.
  }
  
  \Fn{Dispatch(i):}{
    $F$($D$,$W$): Initial/Inherit winner track $\Theta_{i}$ with $D$, $W$.
  
  $\Theta_{i}^{0}$ $\leftarrow$ $F$($D_{i}$,$W_{i}$);
  $\Theta_{i}^{1}$ $\leftarrow$ $F$($D_{i}+S_{d}$,$W_{i}$);
  $\Theta_{i}^{2}$ $\leftarrow$ $F$($D_{i}$,$W_{i}+S_{w}$);\\
  Sends $\Theta_{i}^{0}$, $\Theta_{i}^{1}$, $\Theta_{i}^{2}$ to $Trial_{0}$, $Trial_{1}$, $Trial_{2}$ seperately\;
  Parallel: Client\_training(i,k).
  }
  
  \caption{Cross-device Soft Label Annotating}\label{alg:soft-label}
\end{algorithm}


==> obsolete/fig-def-distribution.tex <==
\begin{figure*}[t]
	\centering
        \includegraphics[width=0.6\textwidth]{figs/def-distribution.pdf}

	%  \vspace{-10pt}
	\caption{We define a new triple tuple (samples, clients, sparsity): noted as ($n$, $\xi$, $\gamma$) to represent the true few show learning (labeled) data distribution. \mwx{N-ways K-shots: way means number of labels, shot means data quantity for each label.}} 
	% \vspace{-15pt}
	\label{fig:def-distribution}
\end{figure*}

==> obsolete/fig-def-fednlp-beta.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.45\textwidth]{figs/def-fednlp-beta.pdf}
	%  \vspace{-10pt}
	\caption{The probability density of quantity of training samples in each of the 100 clients on the 20News dataset with different $\beta$. When $\beta$ is larger, then all clients share more similar numbers of samples; when $\beta$ is smaller, then the range of the quantity is much wider — i.e., the larger differences between clients in terms of their sizes of datasets.} 
	% \vspace{-15pt}
	\label{fig:def-fednlp-beta}
\end{figure}

==> obsolete/fig-def-fsl-distribution.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.45\textwidth]{figs/def-fsl-distribution.pdf}
	%  \vspace{-10pt}
	\caption{Different data distribution for FSL. \mwx{Should be replaced by a system design picture or system implementation comple workflow (including cloud pre-training, labeled data input and fine-tuning on mobile devices.).}} 
	% \vspace{-15pt}
	\label{fig:def-fsl-distribution}
\end{figure}

% \begin{figure}[t]
% 	\centering
% 	 \includegraphics[width=0.27\textwidth]{figs/design-adapter-arch.pdf}
% 	 \vspace{-5pt}
% 	\caption{The structure of adapters used.} 
% 	\vspace{-10pt}
% 	\label{fig:design-adapter-arch}
% \end{figure}


==> obsolete/fig-def-gamma.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.4\textwidth]{figs/def-gamma.pdf}
	%  \vspace{-10pt}
	\caption{Visualizing the labeled data sparsity on \texttt{YAHOO}~\cite{zhang2015character} with  $n$=1024, $\xi$=32, $\gamma$ being {$10^{n}$, n=-3,-2,..,2}. Each sub-figure is a 32$\times$10 matrix, where 32 is the number of clients and 10 is the number of labels. 
	The intensity of each cell represents the number of labeled samples for a specific label in the client-side local data.} 
	% \vspace{-15pt}
	\label{fig:def-gamma}
	\vspace{-10pt}
\end{figure}


==> obsolete/fig-eval-augmentation.tex <==
\begin{figure}[t]
	\centering

    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-augmentation-agnews.pdf}
        \subcaption{AGNEWS}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.23\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-augmentation-agnews.pdf}
        \subcaption{Dataset 2}
    \end{minipage}
	%  \vspace{-10pt}
	\caption{Using unlabeled data for augmentation via soft label inferring.} 
	% \vspace{-15pt}
	\label{fig:def-eval-augmentation}
\end{figure}

==> obsolete/fig-eval-gain-gap.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}[b]{1\textwidth}
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_roberta-large.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_roberta-large.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_roberta-large.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_roberta-large.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{Roberta-Large \mwx{datapoints for Usable accuray instead of fixed 0.1\%.}}
    
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_roberta-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_roberta-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_roberta-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_roberta-base.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{(Roberta-Base)}

    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_bert-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_bert-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_bert-base.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_bert-base.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{(BERT-Base)}

    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_agnews_albert-base-v2.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_mnli_albert-base-v2.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yelp-full_albert-base-v2.pdf}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-gain_gap_yahoo_albert-base-v2.pdf}
        \end{minipage}
    \end{minipage}
    \subcaption{(ALBERT-BASE-V2)}
\end{minipage}
    \caption{Time-to-accuracy throughout a training session. FedPrompt speeds up model convergence significantly. Model is BERT. Sample data: 40. \mwx{cut x-axis to 100 iters}}    \label{fig:eval-gain-gap}
%    \caption{The time-to-accuracy of \sys and baselines with base BERT model.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    
\end{figure*}

% \begin{table*}[]
%     \footnotesize
%     \begin{tabular}{|l|ll|ll|ll|ll|}
%     \hline
%              & \multicolumn{2}{c|}{TC (20news)}    & \multicolumn{2}{c|}{TC (agnews)}   & \multicolumn{2}{c|}{TC (semeval)}   & \multicolumn{2}{c|}{ST (onto)}       \\ \hline
%     Methods & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup \\ \hline
%     Origin   & \multicolumn{1}{l|}{26.70} & 1      & \multicolumn{1}{l|}{44.49} & 1.00  & \multicolumn{1}{l|}{260.67} & 1.00  & \multicolumn{1}{l|}{1034.31} & 1.00  \\ \hline
%     Freeze   & \multicolumn{1}{l|}{7.10}  & 3.76   & \multicolumn{1}{l|}{14.02} & 3.17  & \multicolumn{1}{l|}{105.39} & 2.47  & \multicolumn{1}{l|}{649.47}  & 1.59  \\ \hline
%     Adaptive & \multicolumn{1}{l|}{0.18}  & 150.40 & \multicolumn{1}{l|}{0.67}  & 66.78 & \multicolumn{1}{l|}{2.63}   & 99.13 & \multicolumn{1}{l|}{33.60}   & 30.78 \\ \hline
%     \end{tabular}
%     \caption{Network Traffic Save}
%     \label{tab:eval-communication}
%     \end{table*}

==> obsolete/fig-eval-local-fsl.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[b]{0.3\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-local-fsl-performance.pdf}
        \subcaption{Performance}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.2\textwidth}
        \includegraphics[width=0.98\textwidth]{figs/eval-local-fsl-distribution.pdf}
        \subcaption{Distribution}
    \end{minipage}
    \caption{Local prompt learning performance. (a) N sample(s) per client; (b) Different samples per client performance after 1 iteration training. Local epoch is 10, Clients in total is 10, dataset is \texttt{AGNEWS}, Model is BETR, Train bs is 4.}
    \label{fig:eval-local-fsl}
\end{figure}

==> obsolete/fig-eval-model.tex <==
\begin{figure}[t]
	\centering
        \includegraphics[width=0.5\textwidth]{figs/eval-models-all.pdf}

	%  \vspace{-10pt}
	\caption{FedPET convergence performance with different models and datasets. 0.1\% labeled data uniformly distributed in 32 clients.} 
	% \vspace{-15pt}
	\label{fig:eval-model}
\end{figure}

==> obsolete/fig-eval-performance-datapoint.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/eval-overall-agnews.pdf}
            \subcaption{\texttt{AGNEWS}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1.83\textwidth]{figs/eval-overall-mnli.pdf}
            \subcaption{\texttt{MNLI}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/eval-overall-yahoo.pdf}
            \subcaption{\texttt{YAHOO}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=1\textwidth]{figs/eval-overall-yelp-full.pdf}
            \subcaption{\texttt{YELP} }
        \end{minipage}
    \end{minipage}
    
    \caption{Average accuracy and standard deviation for AUG-FedPrompt across data scales. FedCLS stands for the vanilla federated fine-tuning. Full-set stands for fine-tuning on the full labeled data.}
    \label{fig:eval-performance-datapoint}
    \vspace{-10pt}
\end{figure*}


==> obsolete/fig-eval-performance-gain.tex <==
% \begin{figure}[t]
% 	\centering
%     \begin{minipage}[b]{0.23\textwidth}
%         \includegraphics[width=0.98\textwidth]{figs/eval-performance-gain.pdf}
%         \subcaption{AGNEWS}
%     \end{minipage}
%     ~
%     \begin{minipage}[b]{0.23\textwidth}
%         \includegraphics[width=0.98\textwidth]{figs/eval-performance-gain.pdf}
%         \subcaption{Dataset 2}
%     \end{minipage}
% 	%  \vspace{-10pt}
% 	\caption{Accuracy gain turns more obvious when labeled data is extremely few.} 
% 	% \vspace{-15pt}
% 	\label{fig:def-eval-performance-gain}
% \end{figure}

\begin{figure}[t]
	\centering
        \includegraphics[width=0.3\textwidth]{figs/eval-performance-gain.pdf}

	%  \vspace{-10pt}
	\caption{The conclusion of Figure~\ref{fig:eval-performance-overall}. Accuracy gain turns more obvious when labeled data reaching the `balance point'. Y-axis=Pet-CLS} 
	% \vspace{-15pt}
	\label{fig:eval-performance-gain}
\end{figure}

==> obsolete/fig-eval-performance-overall.tex <==
\begin{figure*}[t]
	\centering
        \includegraphics[width=0.8\textwidth]{figs/eval-performance-overall.pdf}

	%  \vspace{-10pt}
	\caption{Balance point is different for various datasets. \mwx{Can be moved to appendix.}} 
	% \vspace{-15pt}
	\label{fig:eval-performance-overall}
\end{figure*}

==> obsolete/fig-eval-performance.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-agnews.pdf}
            \subcaption{\texttt{AGNEWS}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-mnli_40.pdf}
            \subcaption{\texttt{MNLI}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-yelp-full_40.pdf}
            \subcaption{\texttt{YELP}}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-performance-yahoo_40.pdf}
            \subcaption{\texttt{YAHOO}}
        \end{minipage}
    \end{minipage}
    
    
    \caption{Time-to-accuracy throughout a training session. FedPrompt speeds up model convergence significantly. Model is BERT. Sample data: 40.}    \label{fig:eval-performance-bert}
%    \caption{The time-to-accuracy of \sys and baselines with base BERT model.}
    % \caption{The performance breakdown of computation and communication time. Note that y-axis is logarithmic.}
    
\end{figure*}

% \begin{table*}[]
%     \footnotesize
%     \begin{tabular}{|l|ll|ll|ll|ll|}
%     \hline
%              & \multicolumn{2}{c|}{TC (20news)}    & \multicolumn{2}{c|}{TC (agnews)}   & \multicolumn{2}{c|}{TC (semeval)}   & \multicolumn{2}{c|}{ST (onto)}       \\ \hline
%     Methods & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup & \multicolumn{1}{l|}{Comm.} & Speedup \\ \hline
%     Origin   & \multicolumn{1}{l|}{26.70} & 1      & \multicolumn{1}{l|}{44.49} & 1.00  & \multicolumn{1}{l|}{260.67} & 1.00  & \multicolumn{1}{l|}{1034.31} & 1.00  \\ \hline
%     Freeze   & \multicolumn{1}{l|}{7.10}  & 3.76   & \multicolumn{1}{l|}{14.02} & 3.17  & \multicolumn{1}{l|}{105.39} & 2.47  & \multicolumn{1}{l|}{649.47}  & 1.59  \\ \hline
%     Adaptive & \multicolumn{1}{l|}{0.18}  & 150.40 & \multicolumn{1}{l|}{0.67}  & 66.78 & \multicolumn{1}{l|}{2.63}   & 99.13 & \multicolumn{1}{l|}{33.60}   & 30.78 \\ \hline
%     \end{tabular}
%     \caption{Network Traffic Save}
%     \label{tab:eval-communication}
%     \end{table*}

==> obsolete/fig-eval-sparsity-new.tex <==

% \begin{figure}[t]
%     \centering
%     \begin{minipage}[b]{0.49\textwidth}
%         \begin{minipage}[b]{0.48\textwidth}
%             \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-gamma-fedpet-yahoo.pdf}
%             \vspace*{-4pt}
%             \subcaption{Impact of $\gamma$}
%         \end{minipage}
%         ~
%         \begin{minipage}[b]{0.48\textwidth}
%             \includegraphics[width=0.95\textwidth]{figs/eval-heatmap-fedpet-yahoo.pdf}
%             \subcaption{Impact of $\xi$}
%         \end{minipage}
%     \end{minipage}
%     \caption{Average accuracy of federated few-shot learning under different data quantity and sparsity. $\gamma$ controls the distribution of labeled data. $\xi$ controls the quantity of clients owing labeled data. When $\gamma$ and $\xi$ grow larger, labeled data will be more evenly distributed, and vice versa. Dataset: \texttt{YAHOO}~\cite{zhang2015character}.}    
%     \label{fig:eval-sparsity-new}
    
% \end{figure}


% \vspace{10pt}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.234\textwidth]{figs/eval-sparsity-gamma-fedpet-yahoo.pdf}
    \vspace{-4pt}
    % \subcaption{Impact of $\gamma$}
    \caption{Average accuracy of federated few-shot learning under different data quantity and sparsity. When sparsity $\gamma$ grows larger, labeled data will be more uniformly distributed, and vice versa. Dataset: \texttt{YAHOO}~\cite{zhang2015character}.}    
    \vspace{-8pt}
    \label{fig:eval-sparsity-new}
    
\end{figure}


==> obsolete/fig-eval-sparsity.tex <==
\begin{figure*}[t]
    \centering
    \begin{minipage}[b]{1\textwidth}
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-gamma-fedpet-yahoo.pdf}
            \subcaption{\texttt{YAHOO} (non-iid)}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-yahoo-alpha-0-seed-42-pattern-0.pdf}
            \subcaption{\texttt{YAHOO} (iid)}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-sparsity-gamma-fedpet-agnews.pdf}
            \subcaption{\texttt{AGNEWS} (non-iid)}
        \end{minipage}
        ~
        \begin{minipage}[b]{0.24\textwidth}
            \includegraphics[width=0.95\textwidth]{figs/eval-heatmap-fedpet-mnli.pdf}
            \subcaption{\texttt{MNLI} (non-iid)}
        \end{minipage}
    \end{minipage}
    
    \caption{(a). Scattered is better under non-iid distribution; (b). More data brings benefit; (c). new dataset; (d) impact of clients. \mwx{maybe just show fewer gamma case. It would be looking better.}}    
    \label{fig:eval-sparsity}
    
\end{figure*}


==> obsolete/fig-intro-framework.tex <==
\begin{figure}[t]
	\centering
	 \includegraphics[width=0.48\textwidth]{figs/intro-framework.pdf}
	%  \vspace{-10pt}
	\caption{Workflow of AUG-FedPrompt . 
	% (1) Labeled data are usually sparsely distributed on mobile devices;
	% (2) Pattern encoding some form of task description are created to convert training samples to cloze questions;
	% (3) Client data cannot be transferred, we introduce FL;
	% (4) We propose a novel FL framework, FedPET, to train a model on the client side and transfer the model to the server side for evaluation.
	} 
	\vspace{-10pt}
	\label{fig:into-framework}
\end{figure}

==> obsolete/header-lin.tex <==
% !TeX root = main.tex

%
%\usepackage{epsf,epsfig,textcomp,amsmath,amssymb,subfigure,cite,moreverb}

%\usepackage[table,xcdraw,dvipsnames]{xcolor} % xzl: if want to use auto gen table from  http://www.tablesgenerator.com

%\usepackage{subfigure}
\usepackage{wrapfig}
\usepackage{comment}
%\usepackage{array}
\usepackage{colortbl}

\usepackage{hyperref}
\def\UrlBreaks{\do\/\do-}

%\usepackage[T1,hyphens]{url}
%\usepackage[colorlinks,urlcolor=blue]{hyperref}
%\usepackage{url}

%\usepackage{times}
\usepackage{color,soul}
\usepackage{graphics}
\usepackage{hyperref}
\usepackage{lipsum}
\usepackage{tikz}
\usepackage{enumitem}	% for fine control of list env
\usepackage{listings} % for code listing

%
\usepackage{booktabs}	% xzl: for fancy tables
\usepackage{lipsum}

\usepackage{capt-of}	% xzl: used to override the ``figure'' and ``table'' in caption.

\usepackage{todonotes}  %xzl: for "missing figures"
\usepackage{subcaption} %xzl: for subfigure. incompatible with package subfig

%\usepackage[color]{showkeys}	 % xzl: comment this out in final draft
%\definecolor{refkey}{rgb}{249,158,26}
\definecolor{refkey}{rgb}{0,0,1}
\definecolor{labelkey}{rgb}{0,0,1}

%\definecolor{labelkey}{rgb}{0,0,1}
%\definecolor{refkey}{rgb}{0,0,1}


% jin: multiple sublistings in a single listing
% ref: https://tex.stackexchange.com/questions/269609/lstlisting-with-sublistings-and-captions-and-floating-environment
\usepackage{cleveref}
\AtBeginDocument{\DeclareCaptionSubType{lstlisting}}
\crefname{sublstlisting}{listing}{listings}
\Crefname{sublstlisting}{Listing}{Listings}

% --- all sorts of math fonts ---
% cf: https://tex.stackexchange.com/questions/58098/what-are-all-the-font-styles-i-can-use-in-math-mode
\usepackage{mathrsfs}	% xzl: for Ralph Smith’s Formal Script Font (rsfs)
\usepackage{amsfonts}
%\usepackage{inconsolata} % xzl: this uses inconsolata for texttt

\usepackage[export]{adjustbox} % xzl: flush figure to left/right

%\usepackage{algorithm,algorithmic,amsmath} % jin: for pseudo code
\usepackage{boldline}					% jin: use boldline in the table

\usepackage{multirow}

%\usepackage[dvipsnames]{xcolor}

%
%%\usepackage[bookmarks, breaklinks=true, colorlinks=true, plainpages = false,
%%  citecolor = blue, urlcolor = blue, filecolor = blue,]{hyperref}
%
%\usepackage[labelfont=bf,font=medium]{caption}
%\usepackage[labelfont=bf,textfont=normalfont]{caption}
%\usepackage{multirow}
%
%\renewcommand\section{\@startsection {section}{1}{\z@}%
%   {-3ex \@plus -1ex \@minus -.2ex}%
%   {1.7ex \@plus.2ex}%
%   {\normalfont\large\bfseries}}
%\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%   {-2ex\@plus -1ex \@minus -.2ex}% used to be -2.5
%   {1ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%\renewcommand\subsubsection{\@startsection{subsubsection}{2}{\z@}%
%   {-1ex\@plus -1ex \@minus -.2ex}%
%   {0.3ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%
%\newcommand\minisection{\@startsection{subsubsection}{4}{\z@}%
%   {1ex\@plus 0ex \@minus 0ex}%
%   {-1.5ex \@plus .2ex}%
%   {\normalfont\normalsize\bfseries}}
%

\newcommand{\textbfit}[1]{\textbf{\textit{#1}}}


% ----------- drawing --------------
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,fill=black,draw,text=white,inner sep=1pt] (char) {#1};}}
		
%%------------Formatting----------
% nb: \paragraph{} is built-in and will affect many things --- 
\newcommand{\Paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	 % used to be 6pt
%\newcommand\paratitle[1]{\textit{\textbf{#1}}}
\newcommand\paratitle[1]{\textit{\textbf{#1}} \hspace{1mm}}
%\newcommand{\Paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	
%\newcommand\itno[1]{({\em #1})}
%\newcommand\itemno[1]{({\em #1})}

% @paragraph seems built-in. 
\renewcommand{\paragraph}[1]{\vskip 3pt\noindent\textbf{#1 }}	 % used to be 6pt

%%%%%%%%%%%%%%%% smitemize %%%%%%%%%%%%%%%%%%%%
%
\newenvironment{smitemize}%
  {\begin{list}{$\bullet$}%
     {\setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{2pt}}}%
  {\end{list}}
%
%%%%%%%%%%%%%%%% custom spacing %%%%%%%%%%%%%%%%%%%%
%
%----------- Comments-----------------
\newcommand\Note[1]{\sethlcolor{yellow} \hl{#1}} % highlighted notes of other colors.
						 % For colors info from xcolor package, check out:
						 % http://en.wikibooks.org/wiki/LaTeX/Colors
\newcommand\Noted[1]{} % remove highlights.

\newcommand\xzlNote[1]{\sethlcolor{yellow} \hl{xzl: #1}} % highlighted notes of other colors.

\definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
\definecolor{mygreen}{HTML}{ADFF2F}
\definecolor{mylightgray}{gray}{0.8}
%\newcommand\jin[1]{\sethlcolor{mygreen} {\color{darkblue}\bf\hl{#1}}}
%\newcommand\jin[1]{\fcolorbox{blue}{white}{\bf\em\color{blue}jin:} {\small\em\color{blue}{\fontfamily{qhv}\selectfont #1}}}
\newcommand\jin[2][]{
	\fcolorbox{blue}{white}{\bf\em\color{blue}jin}
	{\small\em\color{blue}{\fontfamily{qhv}\selectfont \underline{#1} #2}}
}

\newcommand\myfootnote[1]{\textcolor{red}{\footnote{#1}}}

%\renewcommand\thefootnote{\textcolor{red}{\arabic{footnote}}}

%====== for estimating final pages ===== %

% xzl: the one uses package enumitem that can fine tune indent.
% 
% for simplicity, can also use \begin{itemize}[leftmargin=*]
\renewcommand\labelenumi{(\theenumi)}
\newenvironment{myitemize}%
  {\begin{itemize}
	[leftmargin=0cm,
		itemindent=.3cm,
		labelwidth=\itemindent,
		labelsep=0pt,
		parsep=0.0pt,
		topsep=0.5pt,
		itemsep=0.5pt,
		align=left]
  }%
  {\end{itemize}}    

\newenvironment{myenumerate}%
  {\begin{enumerate}
	[leftmargin=.cm,itemindent=.5cm,labelwidth=\itemindent,
		labelsep=0pt,
		parsep=1pt,
		topsep=1pt,
		itemsep=3pt,
		align=left]
  }%
  {\end{enumerate}}    

%====== shortcut for ref ===== %
\newcommand\sect[1]{Section~\ref{sec:#1}}	% NB: does not play well with \note{}        

% -------------------FONTS-------------------
%\newcommand{\scenario}[1]{\textit{#1}}
\newcommand{\scenario}[1]{\texttt{#1}}

%\newcommand{\state}[1]{\textsc{#1}}
%\newcommand{\state}[1]{\texttt{#1}}

\newcommand{\system}[1]{\textsf{#1}}

% texttt will be larger than body text..
%\newcommand{\code}[1]{\texttt{\small{#1}}}	
\newcommand{\code}[1]{\texttt{#1}}	

\newcommand{\queue}[1]{\textit{#1}}
% ----------------------------------------------

%--------------------------------------------------------

\input{terms}

% Remove the copyright block space.
% http://ryanlei.wordpress.com/2012/02/13/latex-remove-the-copyright-space-from-the-acms-sig-alternate-template/
\makeatletter
\def\@copyrightspace{\relax}
\makeatother


==> obsolete/sec-abstract.tex <==
\begin{abstract}
    Transformer-based pre-trained models have become the de-facto solution for NLP tasks.
    % motivates the development of natural language processing (NLP).
    Fine-tuning such pre-trained models for downstream tasks often requires tremendous amount of data that is both private and labeled.
    However, in reality:
    1) such private data cannot be collected and is distributed across mobile devices, and
    2) well-curated labeled data is scarce.
    To tackle those issues, we first define a data generator for federated few-shot learning tasks, which encompasses the quantity and distribution of scarce labeled data in a realistic setting.
    Then we propose AUG-FedPrompt, a \textbf{prompt}-based \textbf{fed}erated learning algorithm that carefully annotates abundant unlabeled data for data \textbf{aug}mentation.
    AUG-FedPrompt can perform on par with full-set fine-tuning with very few initial labeled data.

\end{abstract}

==> obsolete/sec-bkgnd-measurement.tex <==

\subsection{Preliminary Measurements}\label{sec:bkgnd-measurement}

==> obsolete/sec-bkgnd.tex <==
\section{Background and Motivations} \label{sec:bkgnd}

% \input{sec-bkgnd-measurement.tex}


==> obsolete/sec-conclusions.tex <==
\section{Conclusions and Future Work}\label{sec:conclusions}

In this manuscript, we comprehensively define a data generator for federated few-shot learning tasks, encompassing the quantity and sparsity of scarce labeled data.
Then we propose AUG-FedPrompt, a federated learning algorithm that orchestrates prompt learning and soft label-based data augmentation.
AUG-FedPrompt shows competitive performance under various federated few-shot learning settings, including uniform and skewed data distribution for scarce labeled data.

% During our experiments, we find that there are still large amount of unlabeled data could not be correctly annotated.
% Thus we will focus on the sufficient leverage of unlabeled data.
% Digging out the potential of unlabeled data will enable few shot learning to perform on par with full scale fine-tuning, even when labeled data is extremely few.
% Ensemble soft label voting tends to be the hopeful method, while it will introduce huge training redundancy.

At last, we find that AUG-FedPrompt demonstrates its strong performance on top of large-scale pre-trained models.
Fine-tuning those `behemoths' is resource-costly.
The communication of enormous updated model parameters also consumes huge bandwidth resources.
% Soft prompt learning (prompt tuning), as another popular research line of prompt training, will also be elaborately researched in the future.
% They are more complicate to train for convergence.
% And picking hyper-parameters for prompt tuning is non-trivial and highly resource-consuming.
% Anyway, 
In the future, we will develop a system solution to make our AUG-FedPrompt resource-efficient.

==> obsolete/sec-definition.tex <==
\section{Problem Definition} \label{sec:def}




==> obsolete/sec-design.tex <==
\section{AUG-FedPrompt Design}\label{sec:design}
Our system integrates hard PL into FL workflow, i.e., FL local training is via hard PL instead of vanilla fine-tuning which training the extra added CLS.

\subsection{Training Workflow}

\subsection{Usage of unlabeled data}
Dynamically choose those soft labeled data within a certain confidence interval.

\mwx{Formulation:}



==> obsolete/sec-eval-augmentation.tex <==
\subsection{Unlabeled Data Usage} \label{sec:eval-augmentation}

\input{fig-eval-augmentation.tex}

Simply augmenting training dataset via unlabeled data inferring does not bring benefit at all. But \textbf{FedPrompt with limited labeled data still lags behind full data fine-tuning.} That means unlabeled data has numerous potential for digging.

\textbf{Draw a line plot to show the margin between few shot Fedpet training and full dataset finetuning.}

Future work:
(1) How many unlabeled samples are tagged correctly?
(2) Assuming that all unlabeled samples are tagged correctly, how many benefit will be brought?

==> obsolete/sec-eval-cost.tex <==
\subsection{System Cost}


Performance of various models, shown in Figure~\ref{fig:eval-model}.

\mwx{Expected conclusion:} Large-scale foundation model is needed to take full advantage of prompt learning. 

\mwx{Show the runtime that arriving the 90\% of full-set accuracy.} Instead of the runtime line because the accuracy gap will confuse the reviewers.

Mobile device: Jetson TX2.

Latency and peak memory of different foundation models.

\mwx{Eval the impact of models.}
BERT: some datasets perform bad. But whether it can caused by the origin BERT feature instead of FedPET.
That is to say, those dataset perform bad on BERT even fine-tuned on full dataset.

Roberta: good performance consist with prior literature~\cite{schick2020exploiting, scao2021many, schick2022true}.
While its memory, latency is extremely high.

MobileBERT, DistilBERT, etc.
\begin{itemize}
    \item Energy exps: per-device energy consumption at average till convergence (bar plot).
    
    \item Network exps: per-device network cost at average till convergence (bar plot).
    
    \item Memory exps.
\end{itemize}

Though local prompt training is quick. 
Overall vanilla FedPrompt system cost should be still extremely high.
Because the whole model needs to be transferred, communication cost will be high.



==> obsolete/sec-eval-gain-gap.tex <==
% \subsection{Gain and Gap}  \label{sec:eval-gain-gap}

% \mwx{Will be merged to Section $\S$\ref{sec:eval-performance}}

% \textbf{Prompt learning performs better than vanilla fine-tuning.} Uniform few show learning results have been shown in Figure~\ref{fig:eval-gain-gap}.

% \input{tab-eval-todo.tex}

==> obsolete/sec-eval-gamma.tex <==
\subsection{Impact of Data Augmentation}  \label{sec:eval-gamma}
\input{tab-eval-softlabel.tex}
\textbf{AUG-FedPrompt enhances FedPrompt performance when labeled data is skewed distributed.}
As shown in Table~\ref{tab:eval-softlabel}, FedPrompt without data augment shows competitive performance when labeled data is uniformly distributed on clients.
While skew distribution of labeled data will hurt FedPrompt performance significantly.
For example, FedPrompt performance degrades to 41.8\% on \texttt{YHAOO} when 256 labeled data is skewed distributed on 32 clients.
Considering that skewed distribution is common in real-world, we integrate AUG-FedPrompt with data augmentation to mitigate the performance degradation.

The intuition of prompts is that they introduce a task description in natural language, it helps task-specific fine-tuning perform well even with few training points.
% The main benefit of prompting, rather than compute efficiency, is data efficiency.
This rationale paves the way for the efficiency of our cross-device soft label inferring.
AUG-FedPrompt helps to label more data correctly at the early stage of training.
Together with our samples filter for annotated data, AUG-FedPrompt makes unlabeled data seldom hurt.
For example, we annotate 100 unlabeled data on each client involved in per round for \texttt{AGNEWS}.
The average annotating accuracy of unlabeled data in the first three rounds is 92.5\%.
The inference accuracy will further increase along with the FL training moves on, reaching 95.3\% at the convergence round.
Those `nail' data, about 5 out of 100 in total, is hard to be correctly annotated and filtered out.
Fortunately, we observe that they do not affect the model convergence as shown in Table~\ref{tab:eval-softlabel}.
After cross-device soft label inferring, AUG-FedPrompt performs on par with full-set fine-tuning and greatly outperforms vanilla few-shot fine-tuning, reaching a usable accuracy with scarce labeled data on local.




==> obsolete/sec-eval-local-fsl.tex <==
\subsection{Local Prompt Learning Performance}

\input{fig-eval-local-fsl.tex}
Few samples can make such a big diff. There are there possible reasons:
1. learning rate is too large, some clients are witnessing overfitting 
2. local training epoch is too big, now it is 10 epochs before aggregation
3. pre-trained models maybe has ``data affinity". Clients owing data prefered by pre-trained models tend to achieve better accuracy. In addition, some data has better quality than others~\mwx{ref}.



==> obsolete/sec-eval-performance.tex <==
\subsection{AUG-FedPrompt Performance across Data Scales}  \label{sec:eval-performance}


\textbf{AUG-FedPrompt enjoys a substantial advantage on each task.}
As shown in Fig.~\ref{fig:eval-performance-datapoint}, we compare our AUG-FedPrompt performance with FedCLS, i.e., the vanilla federated fine-tuning where a generic classifier layer inserted after pre-trained models is fine-tuned.
Highlighted region shows the accuracy gap between AUG-FedPrompt and FedCLS. 
There are up to 50\%, 25\%, 55\%, 38\% accuracy improvement separately for 4 datasets.
Both approaches improve with more labeled data, but AUG-FedPrompt remains better by a varying amount. 
AUG-FedPrompt reaches 99\% relative performance of full-set with 90\% less training data compared to full-set federated training.
AUG-FedPrompt shows a strong zero-shot inferring capability, i.e., without task-specific fine-tuning, expected from \texttt{MNLI} dataset. 
\texttt{MNLI} dataset may need more labeled data to make the sufficient usage of the prompt to the pre-trained models.
As for a usable accuracy, i.e., 90\% relative performance of full-set training accuracy, AUG-FedPrompt only needs 64, 256, 256 in total for \texttt{AGNEWS}, \texttt{YAHOO} and \texttt{YELP},saving up to 99.9\% training data compared to full-set federated fine-tuning.

==> obsolete/sec-eval-prompt-tuning.tex <==
\subsection{Efficiency of Prompt Tuning} \label{sec:eval-pt}
Prompt tuning claims no more manual searching for hand-make prompt~\cite{lester2021power, liu2021p}. 
And further research shows its great performance on big models~\cite{liu2021gpt}.

First, hyper-parameter space is extremely large for training SOTA prompt tuning. 
It is a hard work to reproduce those excellent results. 
And most of them do not release their trained models~\cite{gu2021ppt}.

Second, even assuming that we are well knowledged with perfect hyper-parameter, it still need more iterations to converge compared to vanilla fine-tuning.
Fine-tuning of prompt embeddings requires even more steps~\cite{liu2021gpt}.
And they could only perform on par with vanilla fed fine-tune instead of outperforming (which we did through hard pt).

\mwx{What's the difference between ~\cite{lester2021power, liu2021p, liu2021gpt}?}

==> obsolete/sec-eval-setup.tex <==
\subsection{Experiment Setup} \label{sec:eval-setup}
\input{tab-eval-datasets.tex}
\input{fig-eval-performance-datapoint.tex}
\paragraph{Dataset and models} 
We perform our evaluation on four  English datasets and manually designed prompts\footnote{We try 6, 2, 6, 4 different prompts for each datasets separately and report the chosen one that performs best.
The verbalizers are the same as previous literature~\cite{schick2020exploiting}.},
 detailed information is shown in Table~\ref{tab:eval-datasets}.
(1) \texttt{AGNEWS}~\cite{zhang2015character} is a news classification dataset. Given headline a and text body b, news needs to be classified as one of the four categories World, Sports, Business or Science/Tech.
(2) \texttt{MNLI}~\cite{williams2017broad} is a sentence understanding dataset. Given text pairs x = (a, b), the task is to find out whether a implies b, a and b contradict each other or neither.
(3) \texttt{YELP}~\cite{zhang2015character} is a restaurant rating dataset. Given a customer's review, text should be estimated on a 1-5 star scale.
(4) \texttt{YAHOO}~\cite{zhang2015character} is a text classification dataset. Given a question a and an answer b, one of ten possible categories needs to be assigned.
We run all experiments with the same pre-trained model, roberta-large (355M parameters) from RoBERTa~\cite{liu2019roberta}, which we load from the transformers~\cite{wolf2019huggingface} library.
% \footnote{ All experiments results shown in this manuscript is taken on Roberta-large. While in our micro-experiments, we test three more models: Roberta-base, Bert-base-uncased and Albert-base. AUG-FedPrompt still outperforms significantly on all datasets besides \texttt{MNLI}. Experiment results are shown in Appendix Fig.~\ref{fig:eval-model}}. 

\paragraph{Hyper-parameters} 
In line with previous observations~\cite{scao2021many}, few-shot fine-tuning performance varies across chosen labeled data considerably. 
We run every experiment 3 times in order to reduce variance.
Unless otherwise stated, we use the recommended set of hyper-parameters from previous work~\cite{schick2020exploiting}: 
mini-batch size as 4; local training iteration as 1; learning rate as 10$^{-5}$; max sequence length as 256.
For careful annotation, we filter out those aggregated models performing worse than the zero-shot model and those soft-labeled data with confidence lower than 0.9.
For the FL configurations at the server side, we follow the prior FedNLP literature~\cite{cai2022autofednlp,lin-etal-2022-fednlp} to select 5 participants by default for each training round.
The fine-tuned models will be collected in the central server and aggregated through \textit{FedAvg} algorithm~\cite{mcmahan2017communication}.



% In addition, we show two unexpected results:
% (1). Few samples can make a big difference under local prompt learning.
% (2). Vanilla soft label inferring of unlabeled data will deteriorate training performance instead of doing a help.

% Finally, we analysis the efficiency of prevalent prompt tuning~\cite{lester2021power, liu2021p}.
% The expected results are two folds, shown in $\S$\ref{sec:eval-pt}



% Baselines:
% (1) fed full data fine-tuning.
% (2) fed few shot fine-tuning.
% (3) fed few shot prompt tuning (soft prompt learning).
% (4) local pet (hard prompt learning).





==> obsolete/sec-eval.tex <==
\section{Evaluation} \label{sec:eval}


In this section, we evaluate the performance of AUG-FedPrompt across data scales.
AUG-FedPrompt significantly outperforms naive federated fine-tuning.
It could perform on par with full-set training while saving up to 99.9\% labeled data.
Apart from data efficiency, AUG-FedPrompt shows great robustness under various practical few-shot scenario regardless of skewed or uniform data distribution. 

\input{sec-eval-setup.tex}
\input{sec-eval-performance.tex}
\input{sec-eval-gamma.tex}





==> obsolete/sec-impl.tex <==
\section{Implementation and Setups}\label{sec:impl}

==> obsolete/sec-intro.tex <==
\section{Introduction}\label{sec:intro}

\paragraph{Federated NLP}
The development of pre-trained models 
% (a.k.a. foundation models~\cite{bommasani2021opportunities})
is overwhelming with the rise of BERT~\cite{devlin2018bert}.
Their deployment~\cite{van2019does,kim2021code, svyatkovskiy2020intellicode, brown2020language} is commonly composed of two-step training:
pre-training and fine-tuning.
% Such a two-step training shows compelling use cases on commodity devices, such as mobile phones, personal laptop and so on.
% samples include sentiment analysis, QA, and auto completion. 
Unlike self-supervised pre-training, fine-tuning is supervised, requiring task-specific tremendous labeled data. 
However, the exploitation of private user data is restricted and even prohibited in some cases by several data protection regulations such as GDPR~\cite{voigt2017eu} and CCPA~\cite{pardau2018california}. 
Recently, federate learning (FL) becomes the de-facto approach to train a model with privacy preserved.
%FL enables large-scale cooperation training without collecting raw training data from mobile device.
As such, federated NLP (FedNLP)~\cite{lin-etal-2022-fednlp,cai2022autofednlp} is now an important topic towards practical NLP applications.


\paragraph{Problem and challenge}
A key obstacle to practical FedNLP is data labeling. 
It's much more difficult to label data on client devices than on centrally collected data~\cite{xu2021limu}.
Lack of sufficient labeled data severely limits the practicality and scalability of FedNLP in real-world NLP applications. 
Therefore, it is important to address the issue of few-shot or even zero-shot FedNLP tasks.
There are very few efforts on this topic~\cite{fan2021federated, chen2018federated}, which still assume a fairly large number (typically $>$1000 in total) of labels that are uniformly distributed across clients.
However, in practice, the labeled data distribution could be skewed across clients, and such skewness would result in a significant drop in the accuracy according to our experiments in $\S$~\ref{sec:related-fl}.

\paragraph{Our solution and contribution}

\noindent (1) To address the lack of labeled data, we first design a comprehensive data generator to simulate the labeled data distribution for few-shot FedNLP tasks. 
In particular, the generator has two meta-parameters: data quantity and sparsity, encompassing all possibilities of scarce labeled data in real-world few-shot learning. 
\iffalse
In this manuscript, we first design a comprehensive data generator to simulate the labeled data distribution for few-shot FedNLP tasks. \yuan{In particular,} the generator has two meta-parameters: data quantity and sparsity, encompassing all possibilities of scarce labeled data in real-world few-shot learning. 
\fi

\noindent (2) To boost its accuracy based on the generated data, we design a data-augmented prompt method, namely AUG-FedPrompt, for practical few-shot FedNLP. AUG-FedPrompt orchestrates prompt learning and soft label-based data augmentation.
Prompt learning~\cite{schick2020exploiting} introduces a task description in natural language.
It helps task-specific fine-tuning achieve high accuracy with very few labeled data samples in FedNLP.
Furthermore, to tackle performance degradation caused by skewed distribution, AUG-FedPrompt leverages enormous and easily accessible unlabeled data.
AUG-FedPrompt annotates those unlabeled data and identifies those high-quality samples with the help of model capacity and annotation confidence.
Those samples are then used for FL training in the next rounds.

\iffalse
\yuan{Afterwards,} we design a data-augmented prompt method, namely AUG-FedPrompt, for practical few-shot FedNLP.
AUG-FedPrompt orchestrates prompt learning and soft label-based data augmentation.
Prompt learning~\cite{schick2020exploiting} introduces a task description in natural language.
It helps task-specific fine-tuning achieve high accuracy with very few labeled data samples in FedNLP.
Furthermore, to tackle with performance degradation caused by skewed distribution, AUG-FedPrompt leverages enormous and easily accessible unlabeled data.
AUG-FedPrompt annotates those unlabeled data and identify those high-quality samples with the help of model capacity and annotation confidence.
Those samples are then used for FL training in the next rounds.
\fi

\noindent (3) Our extensive experiments on four English datasets demonstrate that AUG-FedPrompt can achieve a substantial performance gain (25\%--55\% higher accuracy) over the state-of-the-art FedNLP approaches under various few-shot settings.
Augmentation with unlabeled data enhances AUG-FedPrompt to perform well with highly skewed labeled distribution across clients.
Overall, AUG-FedPrompt can achieve a comparable performance with the state-of-the-art FedNLP approaches with less than 0.1\% labeled data.


==> obsolete/sec-related-fl.tex <==
\section{Preliminaryies and problem setup} \label{sec:related-fl}

\paragraph{Federated NLP Training Procedure}
% In personal computing, the NLP training paradigm naturally maps to the ownership of training data. 
The two NLP training phases, i.e., pre-training and fine-tuning, require data of disparate natures. 
While pre-training is typically done on public text corpora such as Wikipedia articles, 
fine-tuning requires domain-specific samples, such as user reviews, messages, or emails. Especially for mobile computing, the domain-specific samples are collected from end users, and distributed over mobile devices. In addition, protecting privacy also should be considered.
\iffalse
In mobile computing, these samples are generated by end users continually, distributed over mobile devices, and in many cases considered privacy sensitive.
\fi
To fine-tune models on such private, distributed data, 
federated learning is the de-facto approach~\cite{lin-etal-2022-fednlp,cai2022autofednlp}.
Ahead of time, a cloud service distributes a pre-trained model to all client devices. 
In a training session targeting a specific NLP task and domain, a cloud service selects multiple mobile devices to participate in training. 
A device trains a local copy of the model with its private data and sends the model updates to the cloud. 
Having aggregated model updates from multiple devices, the cloud sends an updated model to the devices. 
The training procedure repeats many rounds until the model converges.

\input{fig-def-gamma.tex}

\paragraph{Federated few-shot data generator}
Apart from data privacy, lack of sufficient labeled data is also a crucial question and inherent feature for mobile scenarios, i.e., few-shot learning.
Alike full-set dataset could be non-independent and identically distributed (non-iid), the scarce labeled data is not always uniformly distributed in the real world.
Based on the definition of full-set non-iid partition strategies~\cite{lin-etal-2022-fednlp}, we further define the sparsity of labeled data under federated few shot learning scenario.

We define a new triple tuple ($n$, $\gamma$) to represent the practical few-shot learning training data distribution, where $n$ represents the total numbers of labeled data, $\gamma$ represents the sparsity of labeled data.

The quantity of labeled data in selected clients follows a Dirichlet allocation $z$ $\sim$ Dir$_{\xi}$ ($\gamma$) where $\xi$ is the number of clients owing labeled data\footnote{$\xi$ could be an optional hyper-parameter to strict the maximum of clients owing labeled data.
In this manuscript, we fix $\xi$ as 32 for simplicity.}.
We can then assign labeled data from the global labeled dataset to selected clients based on the distribution $z$, i.e., client$_{i}$ owns labeled dataset $|\mathcal{T}_{i}|$ = $z_{i}$$n$. 
For example, as shown in Fig.~\ref{fig:def-gamma},  we visualize the labeled data sparsity on \texttt{Yahoo}~\cite{zhang2015character} with  $n$=1024, $\xi$=32, $\gamma$ being {$10^{n}$, n=-3,-2,..,2}. Each sub-figure is a 32$\times$10 matrix, the intensity of which represents the labeled samples of a particular label. When $\gamma$ is small ($10^{-3}$, $10^{-2}$, $10^{-1}$), the labeled data will be skewed distributed, i.e., only few clients own labeled data; when $\gamma$=$10^{2}$, labeled data is nearly uniformly distributed on all clients.


\textbf{Performance degradation under skewed distribution}
We show the impact of data sparsity on federated few-shot learning in Fig.~\ref{fig:eval-sparsity-new}.
The convergence performance degrades when sparsity $\gamma$ is turning smaller, i.e., labeled data is more and more skewed distributed.
For example, when labeled data is 1024 in total, uniform distribution ($\gamma$=100) will be 26\% better than thick distribution ($\gamma$=0.001).
The rationale behind this is that under the common non-iid labeled data distribution, single client tends to own more specific kinds of data labels.
Such a skewed distribution of labeled data will lead to unfairness, i.e., aggregated model prefers those specific labels.
After all, skewed distribution of labeled data could result in significant accuracy drop.
More detailed analysis will be presented in Section~\ref{sec:eval-gamma}.

\input{fig-eval-sparsity-new.tex}


==> obsolete/sec-related-fsl.tex <==
\section{Proposed Method} \label{sec:related-fsl}

To address the challenge of labeled data privacy concern and scarcity, this paper proposes AUG-FedPrompt that can leverage massive unlabeled data via federated prompt learning. 
The key rationale is fine-tuning the pre-trained model via prompt learning on client devices.
After local training and federated aggregation, cross-device soft label inferring procedure helps carefully annotating clients' enormous unlabeled data. 

\input{fig-intro-framework.tex}
We describe the training workflow of AUG-FedPrompt in Fig.~\ref{fig:into-framework}.
A public pre-trained transformer-based language model $M$ is transferred to chosen clients.
We assume that each client has access to a tiny training set $\mathcal{T}$ and a much larger set of unlabeled samples $\mathcal{D}$.

For local prompt training, we annotate $T$ as the vocabulary of model $M$, $\_\_ \in T$ as the mask token and $T^*$ as the set of all token sequences.
The sequence of input phrases is $\mathbf{x}=\left(s_1, \ldots, s_k\right)$ where $s_i \in T^*$.
The pattern-verbalizer pair $\mathbf{p}$ includes: 
1) a \textit{pattern} $P: X \rightarrow T^*$ maps inputs $x$ to a cloze question containing a single mask; 
2) a \textit{verbalizer} $v: Y \rightarrow T$ maps each output $y$ to a single token representing its task-specific meaning in the pattern.

The purpose of local prompt training is to derive the probability that y is the correct output of x from the probability that v(y) is the most likely token at the masked position in $P(x)$.
Based on this rationale, we define the conditional probability distribution $s_{\mathbf{p}}$ of $y$ given $x$ as:

\begin{equation}
    s_{\mathbf{p}}(y \mid x)=\frac{\exp q_{\mathbf{p}}(y \mid x)}{\sum_{y^{\prime} \in Y} \exp q_{\mathbf{p}}\left(y^{\prime} \mid x\right)} \label{eq:pet-few}
\end{equation}
where $q_{\mathbf{p}}(y \mid x)=M(v(y) \mid P(x))$ is the probability that $M$ assigns to $v(y)$ in sequence $P(x)$.

For client-side fine-tuning, 
$M$ is fine-tuned on local labeled data $(x, y)$ by minimizing the cross-entropy  between $s_{\mathbf{p}}(y \mid x)$ and y.
For server-side aggregation,
in iteration $i$, client $k$ sends the updated model $M^{i}_{k}$ to the cloud for aggregation:
\begin{equation}
    M^{i}=\frac{\sum^{\xi-1}_{k=0}|\mathcal{T}|M_{k}^{i}}{\sum^{\xi-1}_{k=0}|\mathcal{T}|}
\end{equation}
where $M^{i}$ is the aggregated model and $|\mathcal{T}|$ is the size of training set. 

For data augmentation, $M^{i}$ is transferred to those clients with enormous unlabeled data for soft label inferring.
Each unlabeled example $\hat{x} \in D$ is labeled with soft label $\hat{y}$ based on $s_{\mathbf{p}}(\hat{y} \mid \hat{x})$.
The soft-labeled dataset is used to fine-tune the client-side model in the next iteration.

The resulting soft-labeled dataset could consist of enormous samples with wrong labels.
Directly involving them in the next training iteration will poison the foundation model, which makes it could be even worse than purely using the limited labeled data.
To address this issue, we propose two techniques to filter out those wrong samples and remain the purity of augment dataset:
1) \textbf{Filtering by model capacity.} We filter out those models with low model capacity, i.e., the performance on validation datasets is bad.
2) \textbf{Filtering by confidence.} We filter out those samples with low confidence, i.e., the probability of the most likely label is less than a threshold.
Both capacity and confidence are hyper-parameters.
They can be flexibly adjusted according to different scenarios.

% Those models are potentially harmful for subsequent annotating.
% Thus, we further design a dynamic cross-device soft label inferring algorithm called augment+ to safely choose those data that will not hurt.
% The ``distilled'' soft-labeled dataset is used to train the next iteration's global model.

% \paragraph{Reference writing}
% We briefly review pattern-exploiting training (PET) (Schick and Schütze, 2021a,c), the method we use for instruction-based text classification. At its core, PET combines textual instructions with regular finetuning using labeled samples. To that end, users must specify one or more patterns which convert an input example x into a cloze question so that it can readily be processed by a masked language model (MLM) (Devlin et al., 2019).1 These patterns can take on very different forms; some samples are shown in Figure 2. In addition, users must inform the model about the meaning of all output classes; this is done with a verbalizer that assigns a natural language expression to each output y (see Figure 2, right). We refer to the combination of a pattern and verbalizer as a pattern-verbalizer pair (PVP).


% The fine-tuning mostly follows an FL common practice~\cite{bonawitz2019towards1}.
% In each round, a cloud service (or \textit{aggregator}) selects a fixed number of mobile devices (or \textit{clients}) as participants.
% The model is fine-tuned on each client and the model updates will be uploaded/aggregated on the cloud.
% The aggregation is often lightweight and the cloud resources can be flexibly scaled out, so its time cost could be neglected.
% The fine-tuning speed is mainly bottlenecked by the on-device training and the network transmission.
% The most likely network for FedNLP is WiFi, which is highly unstable and constrained from a hundred Kbps to a few Mbps~\cite{xu2021cloud}.
% Note that FL typically executes in synchronous manner, so the more constrained hardware/network often bottlenecks~\cite{reisizadeh2020straggler}.


==> obsolete/sec-related-pl.tex <==
\subsection{System Model} \label{sec:related-pl}
Prompt learning is first proposed by~\toref. It includes two mainstreams: hard prompt learning (a.k.a discrete prompt learning) and soft prompt learning (a.k.a continuous prompt learning).

\textbf{Hard prompt learning.}

\textbf{Soft prompt learning.}

Homogenization provides powerful leverage but demands caution, as the defects of the foundation model are inherited by all the adapted models downstream. 
Despite the impending widespread deployment of foundation models, we currently lack a clear understanding of how they work, when they fail, and what they are even capable of due to their emergent properties~\cite{bommasani2021opportunities}.

==> obsolete/sec-related.tex <==
%\section{Prompted-based Federated NLP for Real-World Few-Shot Text Classification}\label{sec:related}


\input{sec-related-fl.tex}

\input{sec-related-fsl.tex}

% \input{sec-related-pl.tex}


==> obsolete/tab-eval-datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
    \centering
    \footnotesize
    \begin{tabular}{@{}cc|cc@{}}
    \toprule
    Dataset & Prompt   & Train  & Test    \\ \midrule
    \texttt{AGNEWS}~\cite{zhang2015character}  & a ( \_\_\_\_ ) b    & 120,000    & 7.600  \\
    \texttt{MNLI}~\cite{williams2017broad}    & “a” ? ‖ \_\_\_\_, “b”   & 392,702     & 9,815  \\
    \texttt{YAHOO}~\cite{zhang2015character}   & [ Category: ] a \_\_\_\_ b      & 1,400,000    & 60,000  \\
    \texttt{YELP}~\cite{zhang2015character}    & It was \_\_\_\_. a & 650,000       & 50,000   \\ \bottomrule
    \end{tabular}
    \caption{Evaluation datasets. Each dataset is distributed to 1000 clients. Label quantity of each class follows the non-iid label distribution in~\cite{lin-etal-2022-fednlp} where $\alpha=1$.}
    \label{tab:eval-datasets}
    \vspace{-15pt}
\end{table}

==> obsolete/tab-eval-softlabel.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{@{}cc|cccc@{}}
    
    \toprule
    \multicolumn{2}{c|}{Dataset}            & \texttt{AGNEWS} & \texttt{MNLI} & \texttt{YAHOO} & \texttt{YELP} \\ \midrule
    \multirow{2}{*}{Uniform} & FedCLS   & 66.1$\pm$12.8    & 60.1$\pm$0.4 & 57.6$\pm$1.9  & 54.0$\pm$0.1 \\
                            & FedPrompt     & \textbf{87.0}$\pm$0.8   & \textbf{77.6}$\pm$0.8 & \textbf{66.0}$\pm$0.1  & \textbf{61.9}$\pm$0.7 \\
                            \midrule
    \multirow{3}{*}{Skew}  & FedCLS   & 64.8$\pm$3.1   & 37.7$\pm$5.6 & 24.4$\pm$10.3  & 38.3$\pm$8.8 \\
                            & FedPrompt     & 68.4$\pm$2.4   & 42.4$\pm$5.8 & 41.8$\pm$4.3  & 51.2$\pm$1.8 \\
                            & w/ augment & \textbf{90.2}$\pm$0.5   & \textbf{75.7}$\pm$1.2 & \textbf{66.9}$\pm$1.1  & \textbf{58.2}$\pm$2.4 \\ \bottomrule
    \end{tabular}
    \caption{AUG-FedPrompt enhances performance under different few-shot learning settings. 
    FedPrompt stands for AUG-FedPrompt without unlabeled data augmentation.
    Datapoint: 64 for \texttt{AGNEWS}, 1024 for \texttt{MNLI}, 256 for \texttt{YAHOO} and \texttt{YELP}. }
    \label{tab:eval-softlabel}
    \vspace{-10pt}
\end{table}

==> obsolete/tab-eval-todo.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
    \begin{tabular}{llllll}
    \hline
    samples                & Method & \texttt{MNLI}          & \texttt{AGNEWS}        & \texttt{YAHOO}         & \texttt{YELP}          \\ \hline
    \multirow{2}{*}{T=40}   & FedCLS & 0.41          & 0.73          & 0.33          & 0.31          \\
                            & FedPET & \textbf{0.48} & \textbf{0.83} & \textbf{0.52} & \textbf{0.38}  \\ \hline
    \multirow{2}{*}{T=100}  & FedCLS & 0.45          & 0.81          & 0.50          & 0.41          \\
                            & FedPET & \textbf{0.48} & \textbf{0.87} & \textbf{0.65} & \textbf{0.43} \\ \hline
    \multirow{2}{*}{T=1000} & FedCLS & 0.54          & 0.89          & 0.65          & \textbf{0.53}     \\
                            & FedPET & \textbf{0.62} & \textbf{0.91} & \textbf{0.67} & 0.49          \\ \hline
    \end{tabular}
    \caption{\mwx{Comparison of different models.}
    Average accuracy and standard deviation for BERT on \texttt{YELP}, AG's News, \texttt{YAHOO} and \texttt{MNLI} for four training set sizes $|\mathcal{T}|$. Model: BERT-base.}
    \label{tab:eval-todo}
    \end{table}

==> obsolete/terms.tex <==
% !TeX root = main.tex

% -------------------TERMS -------------------

\newcommand{\naive}{\texttt{Naive}}
%\newcommand{\cdm}{\texttt{CD-M}}
%\newcommand{\cdmd}{\texttt{CD-MD}}
%\newcommand{\cdfull}{\texttt{CD-Full}}
\newcommand{\cdm}{\texttt{OursM}}
\newcommand{\cdmd}{\texttt{OursMD}}
\newcommand{\cdfull}{\texttt{OursMDS}}

%\newcommand{\cloudshim}{cloud shim}
%\newcommand{\clientshim}{GPU shim}
\newcommand{\cloudshim}{DriverShim}
\newcommand{\clientshim}{GPUShim}

\newcommand{\secenv}{secure environment}
\newcommand{\unsecenv}{normal environment}

\newcommand{\se}{secure world}
\newcommand{\te}{secure world}
\newcommand{\Te}{Secure world}
\newcommand{\Se}{Secure world}
\newcommand{\nw}{normal world}
\newcommand{\sw}{secure world}

%\newcommand{\sys}{TZGPU}
%\newcommand{\sys}{TinyStack}
%\newcommand{\sys}{CoDryrun}
%\newcommand{\sys}{CODY}
%\newcommand{\sys}{CoDry}
%\newcommand{\sys}{GR-T}
%\newcommand{\systz}{TinyStack-TZ}
\newcommand{\mm}{memory manager}
\newcommand{\rn}{runner}
\newcommand{\disp}{dispatcher}
\newcommand{\rep}{TS-Replayer}

%\newcommand{\gpurip}{GPURnR}
%\newcommand{\gpurip}{GPU replay}
%\newcommand{\gpurip}{GPUReplay}
\newcommand{\gpurip}{GR}

\newcommand{\ir}{IR}

\newcommand{\rnr}{record and replay}
\newcommand{\absmodel}{abstract GPU model}

\newcommand{\ioctl}{\texttt{ioctl}}
\newcommand{\register}{\texttt{reg}}
\newcommand{\dwait}{D$_{wait}$}
\newcommand{\irqwait}{\texttt{irq\_wait}}
\newcommand{\val}{\texttt{val}}

\newcommand{\armtz}{arm trustzone}
\newcommand{\tz}{trustzone}
\newcommand{\TZ}{TrustZone}
\newcommand{\ARMTZ}{ARM TrustZone}
%\newcommand{\tee}{TEE}

\newcommand{\tee}{trusted execution environment}

%% ----------------------------------------------

==> obsolete/todo.tex <==
% \mwx{term: unlabeled data}

% \mwx{Curriculum Learning: from easy samples to difficult ones. Our system: from easy model to difficult ones.}

% \mwx{cloud service or aggregator?}

==> sec-bkgnd-prompt__Felix_Lin_s_conflicted_copy_2022-12-07_.tex <==
% !TeX root = main-Mobisys23-FedPrompt.tex

%\subsection{Prompt Learning} \label{sec:bkgnd-prompt}

$\bullet$ \textbf{Prompt learning}~\cite{liu2021pre} boosts accuracy in fine-tuning NLP models;
it becomes common in NLP training in few-shot scenarios \xzlNote{cite}.
For \texttt{FedFSL}, we find prompts crucial to the early stage of a training sessions, when the model is weak and generating confident pseudo labels can be challenging. 

Without prompts, classic NLP fine-tuning must train a new classification layer given a downstream task. 
Since the layer is trained from scratch, doing so require supervision from substantial labeled data. 
To this end, the insight of prompt learning is that a large foundation model already encodes much knowledge for the downstream task; the model just needs a proper way (``prompts'') to express such knowledge. 


In the example below, we fine-tune a foundation model on \texttt{YELP-F} reviews~\cite{zhang2015character} to classify user satisfaction (1--5, 5 being the highest). 
In a few-shot scenario we have two labeled samples: 
\begin{itemize}
    \item \textit{T$_{1}$} (labeled as 1): I will start by saying we have a nice new deck. That is where the good part ends..
    \item \textit{T$_{2}$} (labeled as 5): Tonya is super sweet and the front desk people are very helpful.
\end{itemize}




We use an example from our experiments to introduce how prompts work.
YELP-Review-Full~\cite{zhang2015character} is a dataset of customer's text review, and the label is the corresponding satisfactory level (1--5 stars).
Assume we have three samples: 

\begin{itemize}
    \item \textit{T$_{1}$} (labeled as 1): I will start by saying we have a nice new deck. That is where the good part ends..
    \item \textit{T$_{2}$} (labeled as 5): Tonya is super sweet and the front desk people are very helpful.
    \item \textit{T$_{3}$} (to infer): Love this place. Never had a bad meal. Good portions and great people..
\end{itemize}

% Furthermore, imagine we are told that the labels of T$_{1}$ and T$_{2}$ are 1 and 5, respectively, and we are asked to infer the correct label for T$_{3}$. 
It is challenging to infer T3 because plausible justifications can be found for both T$_{1}$ and T$_{2}$. 
However, if we know that the underlying task is to identify a satisfactory emotion on a restaurant/people (i.e., a prompt), we can easily assign T$_{2}$'s label 5 to T$_{3}$. \xzlNote{how??}
This illustrates that solving a task from only a few samples becomes much easier when we also have a task description, i.e., a textual explanation that helps us understand what the task is about.

In this case, we can use a prompt as below (in bold):
\begin{quote}
    \small
    "\textbf{It was <MASK>}. Love this place. Never had a bad meal. Good portions and great people.."
\end{quote}

The masked word prediction is mapped to a verbalizer that produces a class (i.e., "1":"terrible", "2": "bad", "3": "okay", "4": "good", "5": "great"). 
Several pattern-verbalizer pairs (PVPs) could be used for a single task, differing either through the pattern, the verbalizer, or both. 
As shown in Figure~\ref{fig:bkgnd-fedfsl}, fine-tuning is done by training the model to produce the correct verbalization. 
The loss is the cross-entropy between the correct answer and the distribution of probabilities amongst the tokens in the verbalizer. 
%We re-use pattern choices from Schick and Schütze~\cite{schick2022true} and select the best one for our main experiment, detailed pattern information could be found in Table~\ref{tab:eval-datasets}.
We refer readers to recent surveys~\cite{liu2021pre, bommasani2021opportunities} for a comprehensive explanation of how prompt learning enhances NLP and its underlying foundations.

\xzlNote{moved}

However, the head layer is not being aware and has not been optimized during pre-training.
Therefore, enormous domain specific labeled data is needed to transfer the knowledge. 
Instead, With hand-crafted linguistic prompts, prompt learning directly extracts the knowledge from a foundational model for downstream language tasks.
%prompt learning is based on language models that model the probability of $text$ directly.
We follow prior work to build the prompt model~\cite{schick2020exploiting} and decompose a prompt into a pattern and a verbalizer. 
The pattern turns the input text into a cloze task, i.e. a sequence with a masked token or tokens that need to be filled.
The verbalizer maps label words to the specific class and is often hand-crafted.


% \cdq{How does inference look like?}
% \mwx{Don't use new symbols. Use the same example above.}
\xzlNote{It is worth noting that...}
To use the fine-tuned model to perform prediction tasks, the original input $T_{3}$ is modified using a prompt $\Omega $ into a textual string template $\dot{T_{3}} $ that has some unfilled slots, and then the language model is used to probabilistically fill the unfilled information to obtain a final string $\hat{T_{3}}$, from which the final output y can be derived.

\input{fig-bkgnd-fedfsl.tex}
\textbf{System model: \texttt{FedFSL} workflow enhanced with above techniques}
We notice that pseudo labeling and prompt learning can well orchestrate and be complimentary to each other:
pseudo labeling heavily relies on the initial model accuracy to get enough, correct labels, for which prompt learning can help;
in turn, prompt learning's ability is limited to the few number of data labels and especially their skewed distribution, for which pseudo labeling can help.
Therefore, we construct an enhanced \texttt{FedFSL} workflow by orchestrating the two techniques atop FedNLP, shown in Fig.~\ref{fig:bkgnd-fedfsl}.
This enhanced workflow is the algorithmic foundation of our future design, and is still dubbed as \texttt{FedFSL} for simplicity.

Our goal is to fine-tune a pre-trained language model $\mathscr{M}$ based on distributed clients' data.
We assume that each client has a tiny training set with labels $\mathcal{T}$ (typically < 10) and a much larger set of unlabeled samples $\mathcal{D}$ (typically > 1000). 
Let $\mathcal{P}$ denotes clients that are available for federated learning and $\mathcal{Q} \subseteqq \mathcal{P}$ denotes clients with gold labels.
% \xzlNote{typical size of T and D??}
In general, \sys consists of two loosely-coupled runtimes residing in a central server.

\begin{itemize}[leftmargin=*]
\item \textbf{Labeling runtime} that continously generates new pseudo labels on clients.
Per $k$ training rounds, it dispatches the global $\mathscr{M}$ to $n$ clients, where the model exhaustively inferences on each local unlabeled data $\hat{x} \in D$ and generates a pseudo label $\hat{y}$.
The data with the top $m$ highest confidence (i.e., $logits$) are added as pseudo labels.
In subsequent training rounds, pseudo labels are treated equally as the gold labels.
The pseudo labels that are generated in previous rounds will also be re-labeled to avoid forgetting events~\mwx{refs}.
The above hyper-parameters $<k,n,m>$ indicate how labeling runtime paces.
\item \textbf{Training runtime} that follows a typical federated learning workflow to fine-tune $\mathscr{M}$.
Per round, the runtime dispatches the global $\mathscr{M}$ to a random set of clients with at least one gold or pseudo labels.
The on-device training is assisted with prompts, provided by the trainers either in hand-crafted or automatic manner~\mwx{refs}.
The updated models are then aggregated (default FedAvg protocol~\mwx{ref}) on the server as the new global $\mathscr{M}$.
The process continues till $\mathscr{M}$ reaches a satisfactory accuracy.
Notably, such a design is compatible with prior FL literature on client/data sampling~\mwx{refs}, privacy enhancements~\mwx{refs: DP, HE}, and communication optimization~\mwx{refs: quant}.
\end{itemize}

%\xzlNote{many of the following details seem less relevant to our contrib. more important questions: what does client data/labels look like (use samples)? who to provide prompts? how does inference look like? what model is trained and how?}

%\xzlNote{I felt pseudo labeling (more important) should go before prompt learning}

\begin{comment}
% We first use pseudo labeling to generate pseudo labels for $\mathcal{D}$.
% \xzlNote{pseudo vs soft labeling -- be consistent}
\cdq{Maybe put this detailed description of pseudo labeling into our design? And leave a high-level description here.}
The pseudo labeling is a decoupled runtime from traditional training that opportunistically expands the data labels for subsequent training.
The cloud server randomly selects a subset of clients as $\mathcal{A}_{i} \in \mathcal{P}$ to generate pseudo labels.
Quantity of initial gold labels on $\mathcal{A}_{i}$ are denoted as $|\mathcal{D}(\mathcal{A}_{i})|$.
Quantity of unlabeled samples on selected clients are denoted as $|\mathcal{T}(\mathcal{A}_{i})|$.
Developer (or server) would pre-define a quantity threshold $m$ to decide quantify of generated pseudo labels for subsequent training, we set it to 100 by default in our preliminary experiments.
If $|\mathcal{D}(\mathcal{A}_{i})| \geqq  m $, gold labels are sufficient for training and pseudo labeling would not be activated.
If not, the could server sends the (pre-trained or aggregated) model $M$ to the selected client $\mathcal{A}_{i}$.
Each client uses the output of $M$ to provide a pseudo label $\hat{y}$ for each unlabeled data $\hat{x} \in D$.
The pseudo labels with the top $m - |\mathcal{D}(\mathcal{A}_{i})|$ highest confidence, i.e. $\max (logits)$, together with the input text are added for subsequent training.
Finally, if client $\mathcal{A}_{i}$ does not have gold labels at initial, i.e., $\mathcal{A}_{i} \notin \mathcal{P}$, we move it to the labeled clients list, i.e., $\mathcal{P}= \mathcal{P}+\mathcal{A}_{i}$.
Server would repeat the above steps multiple time to provide flesh pseudo labels for training continuously.

To better utilize the gold labels and the selected pseudo labels, we propose to use prompt learning to fine-tune the model $\mathscr{M}$.
The fine-tuning mostly follows an FL common practice~\cite{bonawitz2019towards1} except from local prompt training.
Before training starts, the cloud server tries different prompts offline (do zero-shot infer) on pre-trained model $\mathscr{M}$ via large-scale public corpus to find the best prompt for each task.
The best prompt is the one that has the highest accuracy on the server-side test set.
Then server selects a subset of clients with (gold or pseudo) labels as $\mathcal{B}_{i} \in \mathcal{Q}$ to fine-tune the model.
The server sends the best prompt configuration and pre-trained model $\mathscr{M}$ to the selected clients.
The model is fine-tuned on each client with their labeled data, where the pseudo labels and gold labels are treated equally.
The model updates will be uploaded/aggregated on the cloud.
The aggregation is often lightweight and the cloud resources can be flexibly scaled out, so its time cost could be neglected.
\end{comment}

==> sec-bkgnd-pseudo.tex <==
\subsection{Pseudo Label Augmentation} \label{sec:bkgnd-pseudo}

\sys will select those pseudo label with highest confidence, i.e., highest logits output.

Rationale behind pseudo label and theoretical foundation of it, reference:
\begin{itemize}
    \item[1.] Pseudo-Label : The Simple and Efficient Semi-Supervised Learning Method for Deep Neural Networks
    \item[2.] Curriculum Labeling: Revisiting Pseudo-Labeling for Semi-Supervised Learning
    \item[3.] FlexMatch: Boosting Semi-Supervised Learning with Curriculum Pseudo Labeling
\end{itemize}

\textbf{Todo: necessity}
Acc gain under different \texttt{FedFSL} setting.



==> sec-design-overview.tex <==
\subsection{Overview} \label{sec:design-overview}
\input{fig-design-overview.tex}
\sys integrates hard PL into FL workflow, i.e., FL local training is via hard PL instead of vanilla fine-tuning which training the extra added CLS.

\sys is composed of two workflow: training and inference line.
They are decoupled and could run asynchronously.

\cdq{
Elaborate \sys is orthorgonal to traditional FL training optimizations in detail.
}

Framework is shown in Figure~\ref{fig:design-overview} (b). Workflow is shown in Figure~\ref{fig:design-overview} (a). 


==> sec-eval-todo.tex <==
\subsection{Todo} \label{sec:eval-todo}



*New:

1. \textbf{correctness ratio between pseudo label and gold labels.} \\
x-axis: rounds \\
y-axis: correctness ratio \\
legend: [Random, similarity-based sort, representativeness-and-diversity-based vote]

2. \textbf{BitFit+freeze vs. freeze}\\
x-axis: \# of tunable layers \\
y-axis: convergence performance \\
legend: [BitFit+Freeze, Freeze]

3. \textbf{Performance across different datapoints}\\
x-axis: datapoints [0-1024] \\
y-axis: convergence performance \\
legend: [FedCLS, Ours, Ours+]




\paragraph{Effect of early filter}
We noticed that FedBalancer consistently shows high time-to-accuracy performance on all datasets, while the performance of baselines was inconsistent across datasets.
We observed that FedBalancer achieves this improvement of time-to-accuracy performance without sacrificing model accuracy; 
in terms of the final model accuracy, FedBalancer showed improvement over the baselines on all datasets.

Efficient \sys improves the time-to-accuracy performance without sacrificing model accuracy; 
in fact, it improves the accuracy by $XX\% \sim XX\%$.


Baselines:
(1) vanilla FL: train the full model.
(2) freeze FL: freeze the first N layers.

\begin{itemize}
\item End-to-end exps: convergence plots (line plot. X-axis: clock time; Y-axis: testing accuracy).

\item Energy exps: per-device energy consumption at average till convergence (bar plot).

\item Network exps: per-device network cost at average till convergence (bar plot).

\item Ablation study.
\end{itemize}



==> sec-impl.tex <==
\section{Implementation and Setups}\label{sec:impl}

==> tab-eval-baselines.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}c||cc|cc@{}}
    \toprule
    \multirow{2}{*}{Setups} & \multicolumn{2}{c|}{Labeling} & \multicolumn{2}{c}{Training}    \\ \cmidrule(l){2-5} 
                                & Pacing         & Optimization   & Method       & Optimization     \\ \midrule \hline
    \texttt{FedCLS}                      & /            & /              & Head-based   & /                \\ \midrule
    \texttt{FedFSL}                      & Static       & /              & Prompt-based & /                \\ \midrule
    \texttt{FedFSL-BIAS}                 & Static       & /              & Prompt-based & Bias-only tuning \\ \midrule
    \sys                        & Curriculum   & Filtering      & Prompt-based & Depth/Capacity Co-planning     \\ \bottomrule
    \end{tabular}%
    }
    \caption{XX and the baselines. The table summarizes their difference against labeling and training. Head-based means fine-tuning a whole classification layer from scratch. Static pacing means introducing 100 pseudo labels per selected client. Mixed tuning means co-planning the tuned layer depth and capacity.}
    \label{tab:eval-baseline}
    \end{table}

==> todo.tex <==
\mwx{term: unlabeled data}

\mwx{Curriculum Learning: from easy samples to difficult ones. Our system: from easy model to difficult ones.}

\mwx{cloud service or aggregator?}
